Forecasting Smog Clouds With Deep Learning

In this proof-of-concept study, we conduct multivariate timeseries forecasting for the concentrations of nitrogen dioxide (NO2), ozone (O3), and (fine) particulate matter (PM10 & PM2.5) with meteorological covariates between two locations using various deep learning models, with a focus on long short-term memory (LSTM) and gated recurrent unit (GRU) architectures. In particular, we propose an integrated, hierarchical model architecture inspired by air pollution dynamics and atmospheric science that employs multi-task learning and is benchmarked by unidirectional and fully-connected models. Results demonstrate that, above all, the hierarchical GRU proves itself as a competitive and efficient method for forecasting the concentration of smog-related pollutants.

==> sections/discussion.tex <==
In the context of sMAPE scores, gaseous pollutants outperform PM, with NO\tsub{2} being the most accurately predicted.
As for the difference in sMAPE between primary pollutant NO\tsub{2} and secondary pollutant O\tsub{3}, \cite{lee2014assessment} suggest that ambient primary pollutants depend primarily on their respective source emissions whilst secondary pollutants depend not only on the primary emissions but also on the availability of atmospheric oxidants.
Consequently, the prediction of NO\tsub{2} is inherently more tractable than that of O\tsub{3}. The sMAPE scores of NO\tsub{2} of O\tsub{3} reflect this difference in predictability.

Furthermore, the sMAPEs may appear high but require a more nuanced interpretation.
A look at Figure~\ref{fig:results_HGRU_small} gives away that forecasts and ground truths of the gaseous pollutants synchronise to a fair degree.
For the PMs, however, the graphed forecasts are more indicative of an average, showing a lack of retrieval of sharply non-linear patterns, which is especially noticeable for peaks in PM\tsub{10}.
The higher errors of the PMs can be explained by their more ``jagged," more frequently fluctuating temporal evolution being more challenging to capture---see, e.g., Figure~\ref{fig:results_all_combined} and \ref{fig:results_all_combined_two_weeks} for the PMs versus the gaseous pollutants on different timescales.
These issues are less evident for the smoother NO\tsub{2} and O\tsub{3}.

Also, Figure~\ref{fig:results_scatter} showed that all models suffer a negative bias on the testing set.
Despite precautionary measures, the data shifts illustrated in Figure~\ref{fig:ridgeplot_pollutants} hinder the models' performance here.
Figure~\ref{fig:scatter_PM10} and ~\ref{fig:scatter_PM25}, for instance, where the RNNs outperform the MLPs and the hierarchical RNNs particularly excel, would support this by pointing out that the RNNs' long-term memory traces and the hierarchical models' nuanced regularisation make them more robust against a data shift---as opposed to the vanilla MLP.
Possible future refinements to accommodate this problem include diversifying the training date through data augmentation, which was recently applied to weather forecasting by \cite{cheon2024advancing} and generally has been shown to improve robustness and generalisation \citep{bengio2011deep}, or by incorporating models that carry more inductive bias.

Nonetheless, given that the discussed forecasts are performed from 15 km away over one dimension within a three-dimensional complex system, but also given measurement inaccuracies \citep{knmi_readme_pdf} and imprecisely interpolated percentages shown in Appendix~\ref{ap:data_availability}---that both render the data more impure and complicate predictions, the scores evince a compelling degree of accuracy.

Regarding the models individually, a few points stood out.
Firstly, the LSTMs across many training runs proved markedly more resistant to initiating and completing convergence.
Both Table~\ref{table:hyperparams_complete} and the total required epochs for the HLSTM in Figure~\ref{fig:losses_all} highlight this.
This is consistent with the theory in Section~\ref{sec:recurrent_neural_nets}: the GRUs indeed converge faster than the LSTMs---not to mention the lower errors achieved by the GRUs.
Secondly, it stood out that MLPs are performing above expectations, considering they do not have access to long-term pattern retention.
Their accuracy may suggest that the significance of long-term dependencies is overestimated or that the instantaneous nature of weather dynamics is underestimated.
Nonetheless, precisely the improvements that move away from mostly "averaging" forecasts; see the PM predictions in Figure~\ref{fig:results_MLP_med} and Figure~\ref{fig:results_HMLP_med} for example, are the most difficult and demanding.
